Handbook of LHC Higgs Cross Sections: 3. Higgs Properties

This Report summarizes the results of the activities in 2012 and the first half of 2013 of the LHC Higgs Cross Section Working Group. The main goal of the working group was to present the state of the art of Higgs Physics at the LHC, integrating all new results that have appeared in the last few years. This report follows the first working group report Handbook of LHC Higgs Cross Sections: 1. Inclusive Observables (CERN-2011-002) and the second working group report Handbook of LHC Higgs Cross Sections: 2. Differential Distributions (CERN-2012-002). After the discovery of a Higgs boson at the LHC in mid-2012 this report focuses on refined prediction of Standard Model (SM) Higgs phenomenology around the experimentally observed value of 125-126 GeV, refined predictions for heavy SM-like Higgs bosons as well as predictions in the Minimal Supersymmetric Standard Model and first steps to go beyond these models. The other main focus is on the extraction of the characteristics and properties of the newly discovered particle such as couplings to SM particles, spin and CP-quantum numbers etc.

==> YRHXS3_HM.tex <==
\section{High Mass search \footnote{%
    S.~Bolognesi, S.~Diglio, C.~Grojean, E.~Logan, M.~Muehlleitner (eds.);
    plus Authors }}

Plans for YR3:
\begin{enumerate}
\item
High Mass SM search: CPS and Interference 
\end{enumerate}



==> YRHXS3_LM/intro.tex <==
This subsection outlines an interim framework to explore the coupling structure of the recently
observed state.
The framework proposed in this recommendation (\Sref{sec:LM_ir:framework}) should be seen as a continuation of the earlier studies of the LHC sensitivity to the Higgs couplings initiated in Refs.~\cite{Zeppenfeld:2000td, Duhrssen:2003tba, Duhrssen:2004cv, Lafaye:2009vr}, and has been influenced by the works of Refs.~\cite{Hagiwara:1993qt, GonzalezGarcia:1999fq, Barger:2003rs, Manohar:2006gz, Giudice:2007fh, Low:2009di, Espinosa:2010vn, Anastasiou:2011pi}.  It follows closely the methodology proposed in the recent phenomenological works of Refs.~\cite{Carmi:2012yp, Azatov:2012bz, Espinosa:2012ir} which have been further extended in several directions \cite{Cao:2012fz, Boudjema:2012cq, Barger:2012hv, Frandsen:2012rj, Giardino:2012ww, Ellis:2012rx, Draper:2012xt, Azatov:2012rd, Farina:2012ea, Englert:2012cb, Degrande:2012gr, Klute:2012pu, Arhrib:2012yv, Akeroyd:2012ms, Azatov:2012wq, Carena:2012xa, Gupta:2012mi, Blum:2012ii, Chang:2012tb, Chang:2012gn, Low:2012rj, Benbrik:2012rm, Corbett:2012dm, Giardino:2012dp, Ellis:2012hz, Montull:2012ik, Espinosa:2012im, Carmi:2012in, Peskin:2012we, Banerjee:2012xc, Cao:2012yn, Bertolini:2012gu, ArkaniHamed:2012kq, Bonnet:2012nm, Craig:2012vn, Almeida:2012bq, Alves:2012ez, Espinosa:2012in, Accomando:2012yg, Elander:2012fk, Reece:2012gi, Djouadi:2012rh,Dobrescu:2012td} along the lines that are formalized in the present recommendation.
While the interim framework is not final,
it has an accuracy that matches the statistical power of the datasets that the LHC experiments
can hope to collect until the end of the 2012 LHC run
and is an explicit attempt to provide a common ground
for the dialogue in the, and between the, experimental and theoretical communities. 

Based on that framework, a series of benchmark parametrizations are presented in \Sref{sec:LM_ir:benchmarks}.
Each benchmark parametrization allows to explore specific aspects of the coupling structure of the new state.
The parametrizations have varying degrees of complexity,
with the aim to cover the most interesting possibilities that can be realistically tested with
the LHC $7$ and $8\UTeV$ datasets.
On the one hand, the framework and benchmarks were designed to provide a recommendation
to experiments on how to perform coupling fits that are useful for the theory community.
On the other hand the theory community can prepare for results based on the framework discussed in this document.


